Causality Graph of Vehicular Traffic Flow

In an intelligent transportation system, the effects and relations of traffic flow at different points in a network are valuable features which can be exploited for control system design and traffic forecasting. In this paper, we define the notion of causality based on the directed information, a well-established data-driven measure, to represent the effective connectivity among nodes of a vehicular traffic network. This notion indicates whether the traffic flow at any given point affects another point's flow in the future and, more importantly, reveals the extent of this effect. In contrast with conventional methods to express connections in a network, it is not limited to linear models and normality conditions. In this work, directed information is used to determine the underlying graph structure of a network, denoted directed information graph, which expresses the causal relations among nodes in the network. We devise an algorithm to estimate the extent of the effects in each link and build the graph. The performance of the algorithm is then analyzed with synthetic data and real aggregated data of vehicular traffic.

==> LDIG.tex <==
The physical distance and connection of roads have a great impact on the causal underlying graph of sensors. The farther two sensors located, estimation of their connection by statistics looses accuracy since more hidden variables get involved. We can take advantage of locations to simplify the estimation by introducing a localized graph, which can be done in two stages:
\begin{enumerate}
\item (Intra-cluster) Cluster sensors based on physical distance and estimate DIG within each cluster independent of others. 
In example depicted in Fig~\ref{fig:cluster} where clusters are determined, the link between $\bb{X}_3$ to $\bb{X}_2$ for instance would be estimated via $I(\co{\bb{X}_3\to\bb{X}_2}{\bb{X}_{C_1\setminus\{2,3\}}})$.
\item (Inter-cluster) For every pair of clusters, compute heuristically the causality between nodes of each cluster. Consider for example the link between $\bb{X}_8$ to $\bb{X}_3$. To check the cascade and proxy effects, we need to include nodes in the neighborhood of $\bb{X}_8$ or $\bb{X}_3$ in the condition. So we estimate both $I(\co{\bb{X}_8\to\bb{X}_3}{\bb{X}_{C_1\setminus\{3\}}})$ and $I(\co{\bb{X}_8\to\bb{X}_3}{\bb{X}_{C_3\setminus\{8\}}})$, and if both were positive we say a link exists in L-DIG from $\bb{X}_8$ to $\bb{X}_3$.    
\end{enumerate}
%
Note that the separation of nodes in clusters can dramatically affect complexity of the algorithm as it is polynomial in $\abs{\mathcal{X}}$, where the number of nodes in estimation (nodes in each cluster in L-DIG) appear in the power.   
The steps of estimating L-DIG are presented in Algorithm~\ref{alg:LDIG}. 

\begin{figure}[t]
\centering
\begin{tikzpicture}[]
	\tikzstyle{nod} = [draw,thick,circle,inner sep=1pt]
	\tikzstyle{nemp} = [draw=none,fill=none,right]

	\node (C1) [nemp] at (-1.6,1) {$C_1$};
	\node (C2) [nemp] at (5.6,2) {$C_3$};
	\node (C3) [nemp] at (5,-2) {$C_2$};
	
	\node (S1) [nod] at (0,0) {1};
	\node (S2) [nod] at (.6,.6) {2};
	\node (S3) [nod] at (.2,1.5) {3};
	\node (S4) [nod] at (2,1) {4};
	\node (S5) [nod] at (4,-1) {5};
	\node (S6) [nod] at (4.6,-.4) {6};
	\node (S7) [nod] at (4.8,-1) {7};
	\node (S8) [nod] at (4,2) {8};
	\node (S9) [nod] at (4.6,2.6) {9};
	\node (S10) [nod] at (4.6,1.3) {10};
	
	\draw (0.7,0.9) circle (1.6cm);
	\draw (4.2,2) circle (1.4cm);
	\draw (4.2,-1) circle (1.2cm);
	
	\draw [thick,->]  (S9) -- (S8);
	\draw [thick,->]  (S8) -- (S10);

	\draw [thick,->]  (S6) -- (S5);
	\draw [thick,->]  (S7) -- (S5);


	\draw [thick,->]  (S1) -- (S2);
	\draw [thick,->]  (S3) -- (S2);
	\draw [thick,->]  (S4) -- (S3);

	\draw [thick,dashed,->]  (S8) to[bend right=15] (S3);
	\draw [thick,dashed,->]  (S5) to[bend left=15] (S8);
	\draw [thick,dashed,->]  (S10) to[bend left=15] (S6);	
	\end{tikzpicture}	
	\caption{Clustering and estimating L-DIG of Sensors distributed according to physical location. Solid lines are links estimated within each cluster while dashed lines represent links to connect clusters.}
	\label{fig:cluster}
\end{figure} 

\begin{algorithm}[t]
\caption{Detecting Localized Directed Information Graph}
\label{alg:LDIG}
\begin{algorithmic}[1]
 \Procedure{Estimate\_LDIG}{$X_1,X_2,\dots,X_M,C_1,C_2,\dots,C_Q$}
 	\For {every cluster $C_q$}
     \State {$G_{C_q}$ $\gets$ Estimate\_DIG($X_{C_q}$)} \Comment{$G_{C_q}$ is the sub-matrix selected by columns and rows of $G$ corresponding to $C_q$}
    \EndFor
    \For {every cluster $C_q$}
     \For {every node $\bb{X}_j\in C_q$}
      \For {every cluster $C_p\neq C_q$}
       \For {every node $\bb{X}_i\in C_p$} 
        \State {$I_1$ $\gets$ $\hat I(\co{\bb{X}_i\to \bb{X}_j}{\bb{X}_{C_q\setminus\{j\}}})$}
        \State {$I_2$ $\gets$ $\hat I(\co{\bb{X}_i\to \bb{X}_j}{\bb{X}_{C_p\setminus\{i\}}})$}
        \State {$H_1$ $\gets$ $\hat H(\co{\bb{X}_j}{\bb{X}_{C_q\setminus\{j\}}})$}
        \State {$H_2$ $\gets$ $\hat H(\co{\bb{X}_j}{\bb{X}_{C_p\setminus\{i\}}})$}
        \State $G_{i,j} \gets \min\{I_1/H_1, I_2/H_2\}$
       \EndFor
      \EndFor
     \EndFor 
    \EndFor
    \State {$G_\nor$ $\gets$ normalize $G$}
    \State {$DIG \gets (G_\nor>th)$}
    \State\Return {G, DIG}
  \EndProcedure
\end{algorithmic}
\end{algorithm}
